Heterophily-informed Message Passing

Graph neural networks (GNNs) are known to be vulnerable to oversmoothing due to their implicit homophily assumption. We mitigate this problem with a novel scheme that regulates the aggregation of messages, modulating the type and extent of message passing locally thereby preserving both the low and high-frequency components of information. Our approach relies solely on learnt embeddings, obviating the need for auxiliary labels, thus extending the benefits of heterophily-aware embeddings to broader applications, e.g., generative modelling. Our experiments, conducted across various data sets and GNN architectures, demonstrate performance enhancements and reveal heterophily patterns across standard classification benchmarks. Furthermore, application to molecular generation showcases notable performance improvements on chemoinformatics benchmarks.

==> fig/ss_on_gnns/ss_effect_gnn2.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

    \definecolor{crimson2143940}{RGB}{214,39,40}
    \definecolor{darkgray176}{RGB}{176,176,176}
    \definecolor{darkorange25512714}{RGB}{255,127,14}
    \definecolor{forestgreen4416044}{RGB}{44,160,44}
    \definecolor{lightgray204}{RGB}{204,204,204}
    \definecolor{steelblue31119180}{RGB}{31,119,180}
    
    \begin{axis}[
    height=\figureheight,
    legend cell align={left},
    legend style={
      fill opacity=0.8,
      draw opacity=1,
      text opacity=1,
      at={(0.03,0.97)},
      anchor=north west,
      draw=lightgray204
    },
    tick align=outside,
    tick pos=left,
    width=\figurewidth,
    x grid style={darkgray176},
    xmajorgrids,
    xmin=0, xmax=1,
    xtick style={color=black},
    y grid style={darkgray176},
    ymajorgrids,
    ymin=-4.69751810634162, ymax=45.1343667196608,
    ytick style={color=black}
    ]
    \addplot [semithick, steelblue31119180, opacity=0.5, mark=*, mark size=3, mark options={solid}, forget plot]
    table {%
    0.00127190537750721 -1.62162162162161
    };
    \addplot [semithick, darkorange25512714, opacity=0.5, mark=*, mark size=3, mark options={solid}, forget plot]
    table {%
    0.00127190537750721 1.35135135135135
    };
    \addplot [semithick, forestgreen4416044, opacity=0.5, mark=*, mark size=3, mark options={solid}, forget plot]
    table {%
    0.00127190537750721 -0.270270270270268
    };
    \addplot [semithick, crimson2143940, opacity=0.5, mark=*, mark size=3, mark options={solid}, forget plot]
    table {%
    0.00127190537750721 1.35135135135136
    };
    \addplot [semithick, steelblue31119180, opacity=0.5, mark=*, mark size=3, mark options={solid}, forget plot]
    table {%
    0.00936479866504669 22.176500580386
    };
    \addplot [semithick, darkorange25512714, opacity=0.5, mark=*, mark size=3, mark options={solid}, forget plot]
    table {%
    0.00936479866504669 20.6999497597454
    };
    \addplot [semithick, forestgreen4416044, opacity=0.5, mark=*, mark size=3, mark options={solid}, forget plot]
    table {%
    0.00936479866504669 -0.19548495051942
    };
    \addplot [semithick, crimson2143940, opacity=0.5, mark=*, mark size=3, mark options={solid}, forget plot]
    table {%
    0.00936479866504669 5.40297475591867
    };
    \addplot [semithick, steelblue31119180, opacity=0.5, mark=*, mark size=3, mark options={solid}, forget plot]
    table {%
    0.0208237711340189 23.702559576346
    };
    \addplot [semithick, darkorange25512714, opacity=0.5, mark=*, mark size=3, mark options={solid}, forget plot]
    table {%
    0.0208237711340189 21.7122683142101
    };
    \addplot [semithick, forestgreen4416044, opacity=0.5, mark=*, mark size=3, mark options={solid}, forget plot]
    table {%
    0.0208237711340189 -0.123565754633725
    };
    \addplot [semithick, crimson2143940, opacity=0.5, mark=*, mark size=3, mark options={solid}, forget plot]
    table {%
    0.0208237711340189 15.7921447484554
    };
    \addplot [semithick, steelblue31119180, opacity=0.5, mark=*, mark size=3, mark options={solid}, forget plot]
    table {%
    0.0258468985557556 5.12007684918347
    };
    \addplot [semithick, darkorange25512714, opacity=0.5, mark=*, mark size=3, mark options={solid}, forget plot]
    table {%
    0.0258468985557556 5.00480307396733
    };
    \addplot [semithick, forestgreen4416044, opacity=0.5, mark=*, mark size=3, mark options={solid}, forget plot]
    table {%
    0.0258468985557556 -0.172910662824205
    };
    \addplot [semithick, crimson2143940, opacity=0.5, mark=*, mark size=3, mark options={solid}, forget plot]
    table {%
    0.0258468985557556 2.41114313160422
    };
    \addplot [semithick, steelblue31119180, opacity=0.5, mark=*, mark size=3, mark options={solid}, forget plot]
    table {%
    0.0591660216450691 6.21621621621622
    };
    \addplot [semithick, darkorange25512714, opacity=0.5, mark=*, mark size=3, mark options={solid}, forget plot]
    table {%
    0.0591660216450691 4.86486486486486
    };
    \addplot [semithick, forestgreen4416044, opacity=0.5, mark=*, mark size=3, mark options={solid}, forget plot]
    table {%
    0.0591660216450691 -2.43243243243242
    };
    \addplot [semithick, crimson2143940, opacity=0.5, mark=*, mark size=3, mark options={solid}, forget plot]
    table {%
    0.0591660216450691 2.70270270270271
    };
    \addplot [semithick, steelblue31119180, opacity=0.5, mark=*, mark size=3, mark options={solid}, forget plot]
    table {%
    0.0631703287363052 1.84210526315789
    };
    \addplot [semithick, darkorange25512714, opacity=0.5, mark=*, mark size=3, mark options={solid}, forget plot]
    table {%
    0.0631703287363052 3.1359649122807
    };
    \addplot [semithick, forestgreen4416044, opacity=0.5, mark=*, mark size=3, mark options={solid}, forget plot]
    table {%
    0.0631703287363052 0.350877192982468
    };
    \addplot [semithick, crimson2143940, opacity=0.5, mark=*, mark size=3, mark options={solid}, forget plot]
    table {%
    0.0631703287363052 -0.285087719298249
    };
    \addplot [semithick, steelblue31119180, opacity=0.5, mark=*, mark size=3, mark options={solid}, forget plot]
    table {%
    0.0789798200130463 -0.0416987191375617
    };
    \addplot [semithick, darkorange25512714, opacity=0.5, mark=*, mark size=3, mark options={solid}, forget plot]
    table {%
    0.0789798200130463 2.42080006495567
    };
    \addplot [semithick, forestgreen4416044, opacity=0.5, mark=*, mark size=3, mark options={solid}, forget plot]
    table {%
    0.0789798200130463 1.20344249906058
    };
    \addplot [semithick, crimson2143940, opacity=0.5, mark=*, mark size=3, mark options={solid}, forget plot]
    table {%
    0.0789798200130463 7.47211128246079
    };
    \addplot [semithick, steelblue31119180, opacity=0.5, mark=*, mark size=3, mark options={solid}, forget plot]
    table {%
    0.097232960164547 -0.392156862745086
    };
    \addplot [semithick, darkorange25512714, opacity=0.5, mark=*, mark size=3, mark options={solid}, forget plot]
    table {%
    0.097232960164547 4.50980392156862
    };
    \addplot [semithick, forestgreen4416044, opacity=0.5, mark=*, mark size=3, mark options={solid}, forget plot]
    table {%
    0.097232960164547 3.1372549019608
    };
    \addplot [semithick, crimson2143940, opacity=0.5, mark=*, mark size=3, mark options={solid}, forget plot]
    table {%
    0.097232960164547 5.68627450980391
    };
    \addplot [semithick, steelblue31119180, opacity=0.5, mark=*, mark size=3, mark options={solid}, forget plot]
    table {%
    0.126605272293091 0.641077991016747
    };
    \addplot [semithick, darkorange25512714, opacity=0.5, mark=*, mark size=3, mark options={solid}, forget plot]
    table {%
    0.126605272293091 1.36382196815026
    };
    \addplot [semithick, forestgreen4416044, opacity=0.5, mark=*, mark size=3, mark options={solid}, forget plot]
    table {%
    0.126605272293091 0.830951408738267
    };
    \addplot [semithick, crimson2143940, opacity=0.5, mark=*, mark size=3, mark options={solid}, forget plot]
    table {%
    0.126605272293091 -1.90690077582686
    };
    \addplot [semithick, steelblue31119180, opacity=0.5, mark=*, mark size=3, mark options={solid}, forget plot]
    table {%
    0.180130332708359 0.654763344708231
    };
    \addplot [semithick, darkorange25512714, opacity=0.5, mark=*, mark size=3, mark options={solid}, forget plot]
    table {%
    0.180130332708359 5.35883116317856
    };
    \addplot [semithick, forestgreen4416044, opacity=0.5, mark=*, mark size=3, mark options={solid}, forget plot]
    table {%
    0.180130332708359 -1.34155013351027
    };
    \addplot [semithick, crimson2143940, opacity=0.5, mark=*, mark size=3, mark options={solid}, forget plot]
    table {%
    0.180130332708359 2.9631952135689
    };
    \addplot [semithick, steelblue31119180, opacity=0.5, mark=*, mark size=3, mark options={solid}, forget plot]
    table {%
    0.626731038093567 0.22556390977444
    };
    \addplot [semithick, darkorange25512714, opacity=0.5, mark=*, mark size=3, mark options={solid}, forget plot]
    table {%
    0.626731038093567 -0.481203007518816
    };
    \addplot [semithick, forestgreen4416044, opacity=0.5, mark=*, mark size=3, mark options={solid}, forget plot]
    table {%
    0.626731038093567 -0.16541353383458
    };
    \addplot [semithick, crimson2143940, opacity=0.5, mark=*, mark size=3, mark options={solid}, forget plot]
    table {%
    0.626731038093567 1.59398496240601
    };
    \addplot [semithick, steelblue31119180, opacity=0.5, mark=*, mark size=3, mark options={solid}, forget plot]
    table {%
    0.664140343666077 0.134415419731171
    };
    \addplot [semithick, darkorange25512714, opacity=0.5, mark=*, mark size=3, mark options={solid}, forget plot]
    table {%
    0.664140343666077 0.684757798630486
    };
    \addplot [semithick, forestgreen4416044, opacity=0.5, mark=*, mark size=3, mark options={solid}, forget plot]
    table {%
    0.664140343666077 0.284047679431898
    };
    \addplot [semithick, crimson2143940, opacity=0.5, mark=*, mark size=3, mark options={solid}, forget plot]
    table {%
    0.664140343666077 0.557950798884088
    };
    \addplot [semithick, steelblue31119180, opacity=0.5, mark=*, mark size=3, mark options={solid}, forget plot]
    table {%
    0.700173437595367 -0.418181818181795
    };
    \addplot [semithick, darkorange25512714, opacity=0.5, mark=*, mark size=3, mark options={solid}, forget plot]
    table {%
    0.700173437595367 -0.0618181818181962
    };
    \addplot [semithick, forestgreen4416044, opacity=0.5, mark=*, mark size=3, mark options={solid}, forget plot]
    table {%
    0.700173437595367 -0.59636363636365
    };
    \addplot [semithick, crimson2143940, opacity=0.5, mark=*, mark size=3, mark options={solid}, forget plot]
    table {%
    0.700173437595367 16.0327272727273
    };
    \addplot [semithick, steelblue31119180, opacity=0.5, mark=*, mark size=3, mark options={solid}, forget plot]
    table {%
    0.765718162059784 -0.314232902033273
    };
    \addplot [semithick, darkorange25512714, opacity=0.5, mark=*, mark size=3, mark options={solid}, forget plot]
    table {%
    0.765718162059784 -0.942698706099809
    };
    \addplot [semithick, forestgreen4416044, opacity=0.5, mark=*, mark size=3, mark options={solid}, forget plot]
    table {%
    0.765718162059784 -0.0369685767097838
    };
    \addplot [semithick, crimson2143940, opacity=0.5, mark=*, mark size=3, mark options={solid}, forget plot]
    table {%
    0.765718162059784 0.314232902033285
    };
    \addplot [semithick, steelblue31119180, opacity=0.5, mark=*, mark size=3, mark options={solid}, forget plot]
    table {%
    0.772232592105865 0.215686274509808
    };
    \addplot [semithick, darkorange25512714, opacity=0.5, mark=*, mark size=3, mark options={solid}, forget plot]
    table {%
    0.772232592105865 0.0326797385620914
    };
    \addplot [semithick, forestgreen4416044, opacity=0.5, mark=*, mark size=3, mark options={solid}, forget plot]
    table {%
    0.772232592105865 -0.339869281045746
    };
    \addplot [semithick, crimson2143940, opacity=0.5, mark=*, mark size=3, mark options={solid}, forget plot]
    table {%
    0.772232592105865 42.8692810457516
    };
    \addplot [semithick, steelblue31119180, forget plot]
    table {%
    0.5 -4.69751810634162
    0.5 45.1343667196608
    };
    \addplot [semithick, steelblue31119180, forget plot]
    table {%
    0 0
    1 0
    };
    \addplot [semithick, white, opacity=0.5, mark=*, mark size=1.5, mark options={solid,fill=steelblue31119180}]
    table {%
    -1 0
    };
    \addlegendentry{GCN}
    \addplot [semithick, white, opacity=0.5, mark=*, mark size=1.5, mark options={solid,fill=darkorange25512714}]
    table {%
    -1 0
    };
    \addlegendentry{GAT}
    \addplot [semithick, white, opacity=0.5, mark=*, mark size=1.5, mark options={solid,fill=forestgreen4416044}]
    table {%
    -1 0
    };
    \addlegendentry{GraphSAGE}
    \addplot [semithick, white, opacity=0.5, mark=*, mark size=1.5, mark options={solid,fill=crimson2143940}]
    table {%
    -1 0
    };
    \addlegendentry{GIN}
    \end{axis}
    
    \end{tikzpicture}
    

==> fig/visualization_of_triple_channels.tex <==
\begin{tikzpicture}[inner sep=0,outer sep=0,node distance=9mm and 7mm]
    
      % Molecule radius
      \newdimen\R
      \R=.5cm
   
      % Column width
      \newdimen\colwidth
      \colwidth=2.7cm
        
      % Define style of nodes and arrows
      \tikzstyle{atom}=[draw=black!80,fill=white,circle,inner sep=1.7pt]
      \tikzstyle{label}=[text width=.8\colwidth,align=center,font=\bf,anchor=north]      
      \tikzstyle{myarrow} = [draw=black!80, single arrow, minimum height=2em, minimum width=2pt, single arrow head extend=3pt, fill=black!80, anchor=center, rotate=0, inner sep=2pt, rounded corners=1pt]
      \tikzstyle{myarr}=[draw=black,->,shorten >=.1cm,shorten <=.1cm]   
      \tikzstyle{layer}=[rotate=90,font=\tiny,rounded corners=1pt,fill=white,inner sep=4pt,scale=.8]  
      
      % Custom molecule node
      \newcommand{\molecule}[3]{%
        \begin{scope}[shift={(#1)}]
        
        % Define colors
        \foreach \hex [count=\i] in {#3} {
          \xglobal\definecolor{c\i}{HTML}{\hex} 
        }
        
        % Draw hex ring
        \foreach \x [count=\i] in {30,90,...,330} {
           \node[atom,fill=c\i] (a\i) at (\x:\R) {};
        }
        % Draw additional
        \node[atom,fill=c7] (a7) at (210:2\R) {};
        \node[atom,fill=c8] (a8) at (330:2\R) {};  
        
        % Connect
        \foreach \i/\j/\x in {#2} {
          \pgfmathtruncatemacro{\edgecolor}{int(10+10*\x)}
          \pgfmathtruncatemacro{\edgewidth}{int(\x)}  
          \draw[red!\edgecolor,line width=\edgewidth] (a\i) -- (a\j);
        }
        
        \end{scope}}
              
      % Image parts        
      \draw[dashed,black!40,thick] (.5\colwidth,-.5\colwidth) -- (.5\colwidth,-2\colwidth);
      \draw[dashed,black!40,thick] (-.5\colwidth,-.5\colwidth) -- (-.5\colwidth,-2\colwidth);      

      % Labels
      \node[label] at (0,.65\colwidth) {Model input};
      \node[label] at (-\colwidth,.65\colwidth) {3-Aminophenol};      
      \node[label] at (-\colwidth,-.3\colwidth) {Heterophilious channel};
      \node[label] at (0,-.3\colwidth) {Original channel};
      \node[label] at (\colwidth,-.3\colwidth) {Homophilious channel};
      
      % Original molecule
      \node at (-\colwidth,.25\colwidth) {
        \includegraphics[width=.65\colwidth]{fig/Aminophenol3d}};

      % Arrow
      \node[myarrow] (arr) at (-.5\colwidth,.25\colwidth) {};

      % Input
      \molecule{0,.25\colwidth}
        {1/2/3.00,2/3/3.00,3/4/3.00,4/5/3.00,5/6/3.00,6/1/3.00,4/7/3.00,6/8/3.00}
        {16FF16,16FF16,16FF16,16FF16,16FF16,16FF16,1616FF,FF1616}

      % The three columns : First row
      \molecule{-\colwidth,-.75\colwidth}
        {1/2/0.00,2/3/0.00,3/4/0.00,4/5/0.00,5/6/0.00,6/1/0.00,4/7/2.46,6/8/2.46}
        {16FF16,16FF16,16FF16,26FFD7,16FF16,D7FF26,26D7FF,FFD726}
      \molecule{0\colwidth,-.75\colwidth}
        {1/2/3.00,2/3/3.00,3/4/3.00,4/5/3.00,5/6/3.00,6/1/3.00,4/7/3.00,6/8/3.00}
        {16FF16,16FF16,16FF16,1DFF68,16FF16,68FF1D,29FFFF,FFFF29}
      \molecule{\colwidth,-.75\colwidth}
        {1/2/3.00,2/3/3.00,3/4/3.00,4/5/3.00,5/6/3.00,6/1/3.00,4/7/0.54,6/8/0.54}
        {16FF16,16FF16,16FF16,17FF25,16FF16,25FF17,1A43FF,FF431A}

      % The three columns : Second row
      \molecule{-\colwidth,-1.5\colwidth}
        {1/2/0.00,2/3/0.00,3/4/0.54,4/5/0.54,5/6/0.00,6/1/0.54,4/7/0.04,6/8/0.04}
        {34FF18,16FF16,18FF34,22FFA5,32FF32,A5FF22,26D8FF,FFD826}
      \molecule{0\colwidth,-1.5\colwidth}
        {1/2/3.00,2/3/3.00,3/4/3.00,4/5/3.00,5/6/3.00,6/1/3.00,4/7/3.00,6/8/3.00}
        {31FF18,16FF16,18FF31,1CFF65,34FF34,65FF1C,23FFB3,B3FF23}
      \molecule{\colwidth,-1.5\colwidth}
        {1/2/3.00,2/3/3.00,3/4/2.99,4/5/2.99,5/6/3.00,6/1/2.99,4/7/1.20,6/8/1.20}
        {1BFF16,16FF16,16FF1B,19FF3B,1BFF1B,3BFF19,21A0FF,FFA021}



      % The three columns : Third row
      \node at (-\colwidth,-2\colwidth) {\large$\vdots$};     
      \node at (0\colwidth,-2\colwidth) {\large$\vdots$};     
      \node at (1\colwidth,-2\colwidth) {\large$\vdots$};     
      
      % Layers
      \node[layer] at (-.5\colwidth,-.75\colwidth) {Layer 1};
      \node[layer] at (.5\colwidth,-.75\colwidth) {Layer 1};
      \node[layer] at (-.5\colwidth,-1.5\colwidth) {Layer 2};
      \node[layer] at (.5\colwidth,-1.5\colwidth) {Layer 2};
      
      % Connect them by arrows
      \draw[myarr] (0,0\colwidth) -> (0,-.25\colwidth);
      \draw[myarr] (0,0\colwidth) -> (-.2\colwidth,-.2\colwidth);
      \draw[myarr] (0,0\colwidth) -> (.2\colwidth,-.2\colwidth);      
      %\draw[myarr] (0,-.1\colwidth) to[out=180,in=90] (-\colwidth,-.4\colwidth);
      %\draw[myarr,shorten <=0] (0,-.1\colwidth) to[out=0,in=90] (\colwidth,-.25\colwidth);
      
  \end{tikzpicture}
